Shear Viscosity of Clay-like Colloids in Computer Simulations and Experiments

Dense suspensions of small strongly interacting particles are complex systems, which are rarely understood on the microscopic level. We investigate properties of dense suspensions and sediments of small spherical Al_2O_3 particles in a shear cell by means of a combined Molecular Dynamics (MD) and Stochastic Rotation Dynamics (SRD) simulation. We study structuring effects and the dependence of the suspension's viscosity on the shear rate and shear thinning for systems of varying salt concentration and pH value. To show the agreement of our results to experimental data, the relation between bulk pH value and surface charge of spherical colloidal particles is modeled by Debye-Hueckel theory in conjunction with a 2pK charge regulation model.

==> Makefile <==
SHELL=/bin/bash

NAME=shearPaperFinal

.PHONY: all ps force f dvi clean realclean

FILES= \
 $(NAME).tex\
 images/*.eps\

# *.bib\
 *.bst


IMGS := $(wildcard images/*.eps)

PDFIMGS=$(subst eps,pdf,$(IMGS))

all: dvi pdf

$(PDFIMGS): %.pdf: %.eps ;\
 epstopdf $< -o=$@

$(NAME).dvi: $(FILES); \
        latex $(NAME); \
        bibtex $(NAME); \
        latex $(NAME); \
        latex $(NAME)

dvi: $(NAME).dvi

dvipdf: $(NAME).dvi; \
    dvipdf $(NAME)

# pdf: $(FILES); \
    cd images; \
    for f in *.eps; do convert $$f `echo $$f | awk '{gsub("eps","pdf",$$1)}{print $$1}'`; done; \
    cd ..;\
    pdftex $(NAME);\
    rm images/*.pdf

# pdf: $(FILES); \
    latex $(NAME);\
    bibtex $(NAME);\
    vlatex $(NAME);\
    vlatex $(NAME)


pdf: $(PDFIMGS) $(FILES) ; \
        latex $(NAME); \
        bibtex $(NAME); \
        pdflatex $(NAME); \
        pdflatex $(NAME)


ps: $(NAME).dvi; \
    dvips $(NAME); \
    # gv $(NAME).ps

force: ; \
        touch $(NAME).tex; \
        make

f: force ;

submit: *.tex images/*.eps *.bib; \
 cd images; \
 cp job2000k10e7ch15e-3sh7_5e-5.eps fig2a.eps; \
 cp job2000k2e7ch50e-3sh1_5e-4.eps fig2b.eps; \
 cp job2000k30e7ch30e-3sh5e-4.eps fig2c.eps; \
 cp job2000k30e7ch30e-3sh7_5e-4.eps fig2d.eps; \
 cp Energies.eps fig3.eps; \
 cp vprofiles.eps fig4.eps; \
 cp density3mmol.eps fig5a.eps; \
 cp density3mmolShear1000.eps fig5b.eps; \
 cp density25mmol.eps fig5c.eps; \
 cp viscosity.eps fig6.eps; \
 cp finitesize.eps fig7.eps; \
 cp glassy.eps fig8.eps; \
 cp phasediag.eps fig1.eps; \
 cd ..; \
 for f in images/fig*.eps; do echo $$f; epstopdf $$f; done; \
 latex shearPaperSubmission; \
 latex shearPaperSubmission; \
 latex shearPaperSubmission; \
 dvips shearPaperSubmission; \
 pdflatex shearPaperSubmission

clean : ; \
        rm -f *.aux *.log *.lof *.lot *.toc *.bak *.glo *.bbl *.blg $(NAME).ps $(NAME).pdf  images/*.pdf

realclean : ; \
        make clean; \
        rm -f $(NAME).dvi *.ps *.dvi *.pdf images/*.pdf

